Instance As Identity: A Generic Online Paradigm for Video Instance Segmentation

Modeling temporal information for both detection and tracking in a unified framework has been proved a promising solution to video instance segmentation (VIS). However, how to effectively incorporate the temporal information into an online model remains an open problem. In this work, we propose a new online VIS paradigm named Instance As Identity (IAI), which models temporal information for both detection and tracking in an efficient way. In detail, IAI employs a novel identification module to predict identification number for tracking instances explicitly. For passing temporal information cross frame, IAI utilizes an association module which combines current features and past embeddings. Notably, IAI can be integrated with different image models. We conduct extensive experiments on three VIS benchmarks. IAI outperforms all the online competitors on YouTube-VIS-2019 (ResNet-101 43.7 mAP) and YouTube-VIS-2021 (ResNet-50 38.0 mAP). Surprisingly, on the more challenging OVIS, IAI achieves SOTA performance (20.6 mAP). Code is available at https://github.com/zfonemore/IAI

==> Sections/5-limitation.tex <==
\section{Limitation}
Although our IAI paradigm achieve good performance on VIS task, it has two limitations under some cases. The first limitation is the reliance on the segmentation quality of first frame. On one hand, there is no temporal information to assist segmentation in initial frame. On the other hand, as shown in Fig.~\ref{fig:visualization}, the mistakes in the first frame might be propagated to next frames. One possible solution is to utilize multiple frames in the beginning of a video and handle following frames in an online way. Another limitation is the dense scene. Once there is a large quantity of objects in a video, IAI needs much more memory and computation cost to predict IDs and propagate ID information. 
